The Wisdom of the Few? "Supertaggers" in Collaborative Tagging Systems

A folksonomy is ostensibly an information structure built up by the "wisdom of the crowd", but is the "crowd" really doing the work? Tagging is in fact a sharply skewed process in which a small minority of "supertagger" users generate an overwhelming majority of the annotations. Using data from three large-scale social tagging platforms, we explore (a) how to best quantify the imbalance in tagging behavior and formally define a supertagger, (b) how supertaggers differ from other users in their tagging patterns, and (c) if effects of motivation and expertise inform our understanding of what makes a supertagger. Our results indicate that such prolific users not only tag more than their counterparts, but in quantifiably different ways. Specifically, we find that supertaggers are more likely to label content in the long tail of less popular items, that they show differences in patterns of content tagged and terms utilized, and are measurably different with respect to tagging expertise and motivation. These findings suggest we should question the extent to which folksonomies achieve crowdsourced classification via the "wisdom of the crowd", especially for broad folksonomies like Last.fm as opposed to narrow folksonomies like Flickr.

==> JournalOfWebScience-now-abstract.tex <==
A folksonomy is ostensibly an information structure built up by the ``wisdom of the crowd'', but is the ``crowd'' really doing the work? Tagging is in fact a sharply skewed process in which a small minority of ``supertagger'' users generate an overwhelming majority of the annotations. Using data from three large-scale social tagging platforms, we explore (a) how to best quantify the imbalance in tagging behavior and formally define a supertagger, (b) how supertaggers differ from other users in their tagging patterns, and (c) if effects of motivation and expertise inform our understanding of what makes a supertagger. Our results indicate that such prolific users not only tag \emph {more} than their counterparts, but in quantifiably \emph {different} ways. Specifically, we find that supertaggers are more likely to label content in the long tail of less popular items, that they show differences in patterns of content tagged and terms utilized, and are measurably different with respect to tagging expertise and motivation. These findings suggest we should question the extent to which folksonomies achieve crowdsourced classification via the ``wisdom of the crowd'', especially for broad folksonomies like Last.fm as opposed to narrow folksonomies like Flickr.


==> jws-journaldata.tex <==
%We may publish this journal on a per volume basis only, and not on a per issue basis. Will it be problematic to compile articles without an issue number?

\journaltitle      {The Journal of Web Science}
\journalshorttitle {JWS}
\journalurl        {www.nowpublishers.com/JWS}
\journalissnprint  {} %This journal will be an online publication only so there is no print ISSN number.
\journalissnonline {2332-4031}
%\journalcopyrightyear{2010}
\journalaimsandscope{%
Web Science embraces the study of the Web as a vast information network of people and communities. It also includes the study of people and communities by using the digital records of user activity mediated by the Web. An understanding of human behavior and social interaction can contribute to our understanding of the Web, and data obtained from the Web can contribute to our understanding of human behavior and social interaction. Accordingly, Web Science involves analysis and design of Web architecture and applications, as well as studies of the people, organizations, and policies that shape and are shaped by the Web.

To address these diverse goals, \textit{The Journal of Web Science} is inherently interdisciplinary, integrating computer and information sciences, communication, linguistics, sociology, psychology, economics, law, political science, and other disciplines.

\textit{The Journal of Web Science} is unique in the manner in which it brings these disciplines together in creative and critical dialogue. We therefore invite research papers describing original research from all the above disciplines, as well as those that cross traditional disciplinary boundaries.

In order to best serve the community, \textit{The Journal of Web Science} will provide immediate open access to its content. Accepted papers will be published online immediately upon acceptance. The copyright of the published articles stays with the authors. It is free for authors as well as for readers.}

\journalsubmission{%
The \textit{The Journal of Web Science} accepts only electronic submissions. For complete instructions, see www.nowpublishers.com/JWS.}

\journalabstractedin{%
} 
